On Regularity Lemma and Barriers in Streaming and Dynamic Matching

We present a new approach for finding matchings in dense graphs by building on Szemer\'edi's celebrated Regularity Lemma. This allows us to obtain non-trivial albeit slight improvements over longstanding bounds for matchings in streaming and dynamic graphs. In particular, we establish the following results for $n$-vertex graphs: * A deterministic single-pass streaming algorithm that finds a $(1-o(1))$-approximate matching in $o(n^2)$ bits of space. This constitutes the first single-pass algorithm for this problem in sublinear space that improves over the $\frac{1}{2}$-approximation of the greedy algorithm. * A randomized fully dynamic algorithm that with high probability maintains a $(1-o(1))$-approximate matching in $o(n)$ worst-case update time per each edge insertion or deletion. The algorithm works even against an adaptive adversary. This is the first $o(n)$ update-time dynamic algorithm with approximation guarantee arbitrarily close to one. Given the use of regularity lemma, the improvement obtained by our algorithms over trivial bounds is only by some $(\log^*{n})^{\Theta(1)}$ factor. Nevertheless, in each case, they show that the ``right'' answer to the problem is not what is dictated by the previous bounds. Finally, in the streaming model, we also present a randomized $(1-o(1))$-approximation algorithm whose space can be upper bounded by the density of certain Ruzsa-Szemer\'edi (RS) graphs. While RS graphs by now have been used extensively to prove streaming lower bounds, ours is the first to use them as an upper bound tool for designing improved streaming algorithms.

==> dynamic.tex <==
%Let $G= (V,E)$ be any given graph,
%and $A,B\subseteq V$ be any disjoint vertex subsets.
%We write $e(A,B)$ to denote the number of edges between $A,B$.
%If $A,B\neq \emptyset$, we define the {\em density of edges} between
%$A$ and $B$ by
%\begin{align*}
%    d(A,B) := \frac{|E(A,B)|}{|A||B|}.
%\end{align*}
%For a parameter $\gamma \in (0,1)$,
%we say $(A,B)$ is $\gamma$-regular if for every $X\subseteq A$ and
%$Y\subseteq B$ satisfying $|X|\geq \gamma|A|$ and $|Y|\geq \gamma |B|$,
%we have
%\begin{align*}
%    \sizeof{d(A,B) - d(X,Y)} < \gamma.
%\end{align*}
%
%Let $C_0,C_1,\ldots,C_k$ be a partition of the vertex set $V$.
%We say this partition is {\em equitable} if the classes
%$C_1,\ldots,C_k$ all have the same size.
%We will call $C_0$ the {\em exceptional class}.
%We say this partition is $\gamma$-regular if
%both of the following statements are true:
%\begin{enumerate}
%    \item It is equitable and $|C_0|\leq \gamma n$.
%    \item All but at most $\gamma \binom{k}{2}$ of the pairs
%    $C_i,C_j$ for $1\leq i < j \leq k$ are $\gamma$-regular.
%\end{enumerate}
%We will need the following algorithmic version of regularity
%lemma.
%Here $M(n)$ is the time for multiplying two $n\times n$
%matrices with $0,1$ entries.
%\begin{theorem}[\cite{AlonDLRY92}]
%\label{thm:regularityalgo}
%There exists a function
%$Q:\mathbb{R}^{+}\times \mathbb{R}^{+}\to \mathbb{R}^{+}$
%satisfying $\log^* Q(x,y) \leq \poly(x,y)$ for all $x,y$,
%such that,
%given any $n$-vertex graph $G=(V,E)$
%and $\gamma \in (0,1), t\geq 1$,
%one can find in $M(n) Q(t,1/\gamma)$ time
%a $\gamma$-regular partition of $V$
%into $k+1$ classes such that $t\leq k \leq Q(t,1/\gamma)$.
%\end{theorem}

% \sbcomment{Can we turn this into a decomposition to one with parts of the same size?}

% \hl{Indeed, the paper~\cite{AlonDLRY92}
% states their results in terms of equitable partitions.}

In this section, we use the matching cover of \cref{sec:matcover} to prove the following result for the fully dynamic model.

\begin{theorem}\label{thm:dynamicalgo}
There is a randomized, fully dynamic algorithm
that maintains with high probability a $(1-o(1))$-approximate matching
under (possibly adversarial) edge updates.
The algorithm has initialization time
$O(n^{\omega} \log n)$
and worst-case update time $O(n (\log^* n)^{-\Omega(1)})$.
\end{theorem}

We will first show an algorithm with initialization time $O(n^{\omega} \log n)$
and {\em amortized} update time $O(n (\log^* n)^{-\Omega(1)})$,
and then discuss how to make the update time worst-case.

Similar to \cref{sec:matcover},
we fix
$t = (\log^*n)^{\delta}, \gamma = (\log^* n)^{-\delta}$
for some sufficiently small constant $\delta\in(0,1)$
such that we have $Q(t,1/\gamma) \leq \log n$ for the function $Q$ in \cref{thm:regularityalgo}.
Then by \cref{thm:regularityalgo},
%using the current fastest matrix multiplication algorithm~\todo{add citation},
we get that one can find in $O(n^{\omega}\log n)$ time a
$\gamma$-regular partition $C_0,C_1,\ldots,C_k$ of $V$ such that
$(\log^*n)^{\delta} \leq k\leq \log n$.


Also similar to \cref{sec:matcover},
we say a pair $(C_i,C_j)$ of vertex classes is
{\em good} if (i) $1\leq i<j\leq k$, (ii) it is $\gamma$-regular, and
(iii) the density $d(C_i,C_j) \geq 8\gamma$.
We say it is {\em bad} otherwise.
We also say an edge of $G$ is {\em good} if it is between
a good pair $(C_i,C_j)$, and {\em bad} otherwise.
%As in \cref{cl:fewedgespicked},
%we have the following bound on the number of bad edges:
%\begin{proposition}
%The number of bad edges of $G$
%is at most $O(\gamma n^2)$.
%\label{prop:numofbad}
%\end{proposition}
%\begin{proof}
%  \todo{Move to appendix.}
%  We count the number of different types of bad edges separately.
%  \begin{enumerate}
%    \item \textbf{Edges within each class:}
%      The total number is bounded by
%      \begin{align*}
%        \binom{|C_0|}{2} +
%        \sum_{i=1}^{k} \binom{|C_i|}{2}
%        \leq \binom{\gamma n}{2} + k \binom{n/k}{2} <
%        \gamma^2 n^2 + n^2 /k \leq
%        \gamma^2 n^2 +
%        n^2 (\log^*n)^{-\delta}.
%      \end{align*}
%    \item \textbf{Edges between $C_0$ and other $C_i$'s:}
%      The total number is bounded by
%      \begin{align*}
%        \sum_{i=1}^{k} |C_0| |C_i| \leq |C_0| n \leq \gamma n^2.
%      \end{align*}
%    \item \textbf{Edges between sparse $C_i,C_j$'s:}
%      The total number is bounded by
%      \begin{align*}
%        \sum_{0\leq i<j\leq k: d(C_i,C_j) < 8\gamma} |E(C_0,C_i)|
%        \leq 8\gamma n^2.
%      \end{align*}
%  \end{enumerate}
%  Summing up these three upper bounds and noting that
%  $\gamma = (\log^* n)^{\delta}$ finish the proof.
%\end{proof}

In our algorithm,
we will deal with the sparse case and the dense case
separately.
Specifically,
%we fix some constant $\delta' \in (0,1)$,
%and
when the number of edges 
is bounded by $n^2 (\log^* n)^{-\Omega(1)}$,
we will run the Gupta-Peng algorithm~\cite{GuptaP13}
on the entire graph;
otherwise, we run the Gupta-Peng algorithm
on a sparse subgraph that is with high probability a matching cover of the entire graph,
and is obtained by a similar process as the algorithm in \cref{sec:matcover}.
%on a subgraph with $n^2 (\log^* n)^{-\Omega(1)}$ edges
%that is obtained based on a $\gamma$-regular partition
%of the graph.
We formalize our algorithm in \Cref{alg:dynamic}.
We summarize the performance of the Gupta-Peng algorithm
in the following theorem.
\begin{theorem}[Gupta-Peng~\cite{GuptaP13}]
There is a deterministic, fully dynamic algorithm
for maintaining a $(1-\eps)$-approximate matching
with initialization time $O(m_0\eps^{-1})$ and
worst-case update time $O(\sqrt{m} \eps^{-2})$,
where $m_0$ is the number of edges in the initial graph,
and $m$ is the maximum number of edges
in the graph throughout the updates.
\end{theorem}

\begin{Algorithm}\label{alg:dynamic}
  \begin{center}
		A fully dynamic algorithm that maintains a $(1 - o(1))$-approximate matching.
	\end{center}
  
  \vspace{0.3cm}
  
  $t \gets (\log^*n)^{\delta}$, $\gamma \gets (\log^*n)^{-\delta}$
  for some constant $\delta\in(0,1)$
  such that $Q(t,1/\gamma) \leq \log n$.

  \quad

  $\eps \gets 10 (\log^*n)^{-\delta/64}$.

  \quad

\textbf{Sparse regime:}

\begin{enumerate}
    \item Whenever the number of edges exceeds
      $n^2 (\log^* n)^{-\delta/8}$, switch to the dense regime.
    \item Use the Gupta-Peng algorithm to maintain
      a $(1-\eps)$-approximate matching.
    %with $\eps = 10 (\log^*n)^{-\delta/24}$.
\end{enumerate}

\textbf{Dense regime:}

\begin{enumerate}
    \item Whenever the number of edges falls below
    $n^2 (\log^* n)^{-\delta/8}/2$,
    restart the Gupta-Peng algorithm for maintaining a $(1-\eps)$-approximate matching,
    initiate the data structure with the edges of the entire current graph,
    and switch to the sparse regime.
    \item Do the following every $n^{\omega-1}\log^2 n$ updates
      (including before the first update):
    \begin{enumerate}
    \item Run the algorithm in \cref{thm:regularityalgo}
    to obtain a $\gamma$-regular partition
    $C_0,\ldots, C_{k}$ with
    $t = (\log^* n)^{\delta} \leq k\leq Q(t,1/\gamma) \leq \log n$.
    %\label{line:2a}
    \item Let $F\subseteq E$ be
    a subset of edges
    obtained by $F := F_1 \union F_2 \union F_3$ where
    \begin{enumerate}
        \item $F_1$ contains
        the edges between the bad pairs;
        i.e. $F_1:= \Union_{\text{bad}\ C_i,C_j} E\intersect (C_i\times C_j)$
        \item $F_2$ contains
        the edges within each class;
        i.e. $F_2:= \Union_{0\leq i \leq k} E\intersect (C_i\times C_i)$.
        \item $F_3$ is obtained
        by sampling the edges
        between good pairs with probability
        $\frac{10}{\log n}$; i.e.
        $F_3 = \Union_{\text{good}\ C_i,C_j}
        (E\intersect (C_i\times C_j))[\frac{10}{\log n}]$.
    \end{enumerate}
    \item Restart the Gupta-Peng algorithm
        for maintaining a $(1-\eps)$-approximate matching,
        and initialize the Gupta-Peng data structure with the edges in $F$.
        \label{line:2c}
    \end{enumerate}
    \item Upon the insertion of an edge
      $e$, let $F\gets F\union \{e\}$ and insert $e$ into the Gupta-Peng data structure.
    \item Upon the deletion of an edge $e$,
      if $e\in F$, let $F\gets F - \{e\}$ and delete $e$ from the Gupta-Peng data structure;
      otherwise ignore the deletion.
\end{enumerate}
%\end{tbox}

%\caption{A fully dynamic algorithm for maintaining
%  $(1 - o(1))$-approximate matching.
%with $\eps = 10 (\log^*n)^{-\delta/24}$.
%}
%\label{fig:dynamicmatalgo}
\end{Algorithm}

As in \cref{cl:fewedgespicked},
%By the way $F$ is constructed,
%and \cref{prop:numofbad},
we have the following bound on the number of edges
in the Gupta-Peng data structure.

\begin{proposition}
In the dense regime,
the number of edges in the Gupta-Peng data structure
is always at most $O(\gamma n^2)$.
\end{proposition}
This proposition then implies a bound on the amortized
update time of the algorithm.
\begin{proposition}
The amortized update time of
\Cref{alg:dynamic} is
$O(n(\log^* n)^{-\delta/16})$.
\end{proposition}

We then show that the algorithm
maintains a $(1 - o(1))$-approximate matching
with high probability.
For the sparse regime, this directly
follows from the correctness of the Gupta-Peng algorithm.
We thus focus on the dense regime.
To this end, note that
$F_3$ is obtained
by sampling the edges between the good pairs
with probability $\frac{10}{\log n}$, which is larger than the $\log^5 n / n$ sampling rate
in the algorithm for obtaining a matching cover in \cref{sec:matcover}.
Therefore we immediately have \cref{cl:goodpair-sample-nonempty}.
In fact, by a standard application of the Chernoff bound,
we have the following stronger version: % of \cref{cl:goodpair-sample-nonempty}:

\begin{claim}\label{cl:goodpairs}
  W.h.p., it holds for all $X\subseteq C_i, Y\subseteq C_j$ such that $(C_i, C_j)$ a good pair, $|X|\geq \gamma |C_i|$, and $|Y|\geq \gamma |C_j|$ that  $F_3(X,Y) > n^2 / \log^6 n$.
\end{claim}

This claim, coupled with the fact that we only use $F_3$ for $n^{\omega-1} \log^2 n < n^2 / \log^6 n$ updates, 
means that for all $X,Y$ satisfying the requirements of the claim, we have $F_3(X,Y)\neq \emptyset$ always.
Note that this is true even if the updates are chosen {\em adversarially}.
As a result, by a same analysis as we did in the proof of \cref{lem:whpmatchingcover},
we have that the edges in the Gupta-Peng data structure always form
an $\alpha$-matching cover for some $\alpha = \Theta((\gamma \log(1/\gamma))^{1/3}) \leq O((\log^* n)^{-\delta/6})$.
Now the correctness
follows by observing that the maximum matching size of $G$ is $\Omega(n (\log^* n)^{-\delta/8})$ in the dense regime.


%For the dense regime, the correctness follows from that
%the subgraph $G[F]$ is a $O((\log^* n)^{-\delta/6})$-matching cover of $G$,
%as we show in the proposition below,
%and the observation that the maximum matching size of $G$ is $\Omega(n (\log^* n)^{-\delta/8})$ in the dense regime.
%The following lemma shows a property of the subgraph $G[F]$.
%and prove the correctness for
%any $\eps \geq 10/(\log^* n)^{\delta/3}$.

%We first show that
%any good pair $C_i,C_j$ remains
%regular throughout the $n^{\omega-1}\log^2 n$ updates.

%\begin{lemma}
%If $C_i,C_j$ is a good pair at the time we compute
%the $\gamma$-regular partition,
%then throughout
%the following $n^{\omega-1}\log^2 n$ updates,
%$C_i,C_j$ is $2\gamma$-regular
%and has density $d(C_i,C_j)\geq 4\gamma$.
%\end{lemma}

%\begin{proposition}%[of \cref{lem:xy}]
%  \label{cor:matcover}
%  At any given point of the dense regime,
%  $G[F]$ is an $\alpha$-matching cover of $G$ with high probability
%  for $\alpha = \Theta((\gamma \log(1/\gamma))^{1/3}) \leq O((\log^* n)^{-\delta/6})$.
%\end{proposition}
%Note that the proof of \cref{cor:matcover} is very similar to that of \cref{lem:whpmatchingcover},
%but we include it for completeness.
%The proof will rely on the following lemma, which shows a similar guarantee for edges between good $C_i,C_j$ pairs
%as~\Cref{cl:goodpair-sample-nonempty}.
%\begin{lemma}
%If $C_i,C_j$ is a good pair at the time we compute
%the $\gamma$-regular partition,
%then with high probability,
%throughout
%the following $n^{\omega-1}\log^2 n$ updates,
%we have $F(X,Y)\neq \emptyset$ for any $X\subseteq C_i, Y\subseteq C_j$
%satisfying $|X|\geq \gamma |C_i|,|Y|\geq \gamma |C_j|$.
%\label{lem:xy}
%\end{lemma}
%
%We now first show how \cref{lem:xy} implies
%\cref{cor:matcover}, and then prove \cref{lem:xy}.
%
%\begin{proof}[Proof of \cref{cor:matcover} using \cref{lem:xy}]
%  We show that for any matching $M$ of size $\alpha n$ in $G$, there exists an edge in $F$
%  between the vertices matched by $M$.
%  If $M$ has an edge that is not between a good $C_i,C_j$ pair,
%  then such an edge must belong to $F$, which
%  satisfies the matching cover requirement.
%  We thus focus on $M$'s that only contains edges between good $C_i,C_j$ pairs.
%
%  Now consider the meta graph of $k$ supernodes $1,\ldots,k$, where node $i$ represents vertex class $C_i$.
%  Define a fractional matching $\b{x}$ in this meta graph where $x_{ij}$ is the fraction of the vertices in $C_i$
%  that are matched to $C_j$ by $M$.
%  Note that by our assumption on $M$,
%  $x_{ij}\neq 0$ only if $C_i,C_j$ is a good pair.
%  Also since $M$ is of size $\alpha n$,
%  and $\sum_{i=1}^{k} |C_i| \leq n$,
%  we have $|\b{x}|\geq \alpha k$.
%
%  Now by applying \cref{lem:fractionalmatching}
%  with $\eps$ satisfying $\frac{\eps^3}{12 \ln(1/\eps)} = \gamma$
%  (i.e. $\epsilon = \Theta((\gamma \log(1/\gamma))^{1/3})$),
%  we get another fractional matching $\b{y}$ with the following properties
%  \begin{enumerate}[label=(Y\arabic*)]
%    \item For any $i \in [k]$, $y_i \leq x_i$.
%    \item $\supp(\b{y}) \subseteq \supp(\b{x})$.
%    \item For any $i, j \in [k]$ either $y_{ij} = 0$ or $y_{ij} \geq \gamma$,
%    \item $|\b{y}| \geq |\b{x}| - \epsilon k.$
%  \end{enumerate}
%  By choosing a suitable value of $\alpha = \Theta((\gamma \log(1/\gamma))^{1/3})$,
%  we have $|\b{y}| > 0$.
%  Thus, there must exist a good $C_i,C_j$ pair for which $y_{ij} \geq \gamma$.
%  This coupled with \cref{lem:xy} finishes the proof.
%\end{proof}
%
%\begin{proof}[Proof of \cref{lem:xy}]
%  Consider fixing a pair of $X\subseteq C_i, Y\subseteq C_j$
%  satisfying $|X|\geq \gamma |C_i|,|Y|\geq \gamma |C_j|$ for a good pair $C_i,C_j$,
%  and assume we are at a point where we just executed Lines~\ref{line:2a}-\ref{line:2c}.
%  Since $C_i,C_j$ is good, we know that $d(C_i,C_j) \geq 8\gamma$ and
%  $d(X,Y) \geq d(C_i,C_j) - \gamma \geq 7\gamma$.
%  Thus, the number of edges between $X,Y$ in $E$ is
%  \begin{align*}
%    |E(X,Y)| \geq & d(X,Y) |X| |Y| \\
%    \geq & 7\gamma (\gamma |X|) (\gamma |Y|) \\
%    \geq & 7 \gamma^3 (n/k)^2 \\
%    \geq & 7 (\log^* n)^{-3\delta} (n/\log n)^2 \\
%    \geq & 7 n^2 / \log^5 n.
%  \end{align*}
%  Since in obtaining $F$ we sample edges between $C_i,C_j$ with probability $n^{-0.1}$,
%  using a Chernoff bound,
%  with probability at least $1 - e^{-n^{1.9}(\log^{-5} n)/1000}$,
%  we have
%  \begin{align}
%    |F(X,Y)| \geq n^{1.9}\log^{-5} n.
%    \label{eq:fxylb}
%  \end{align}
%  Taking a union bound over all desired $X,Y$ pairs,
%  we have~(\ref{eq:fxylb}) for all $X,Y$'s.
%  The lemma then follows by noting that
%  $n^{\omega-1}\log^2 n < n^{1.9}\log^{-5} n$.
%\end{proof}

%The correctness of the dense regime then follows from
%the following corollary of \cref{lem:xy}.

\def\gg{G_{\mathrm{good}}}
\def\mg{M_{\mathrm{good}}}

%\begin{lemma}
%Let $M^*$ be a maximum matching in $G$.
%The subgraph $G[F]$ has a matching $M'$
%such that $|M'|\geq |M^*| - n/(\log^*n)^{\delta/3}$.
%\end{lemma}
%\begin{proof}
%Let $\mg^*$ denote the edges in $M^*$ that
%are between good $C_i,C_j$ pairs.
%Let $\gg$ be the subgraph induced by the edges
%between good $C_i,C_j$ pairs,
%and let $\gg[F]$ be $\gg$ induced by edge slots in $F$.
%We show that there exists
%a matching $\mg'$ in $\gg[F]$ such that
%$|\mg'| \geq |\mg^*| - n/(\log^*)^{\delta/3}$.
%
%Let us first view $\mg^*$ as a {\em fractional} matching
%(call it $M_f$)
%in the meta graph $H$, which consists of $k$ supernode,
%with the $i^{\mathrm{th}}$ supernode representing
%$C_i$. The fraction on the edge $(i,j)$
%is then given by the number of matching edges between
%$C_i,C_j$ divied by $|C_i|$, i.e.
%$\frac{|\mg^*\intersect (C_i\times C_j)|}{|C_i|}$.
%For each $C_i$, we use $d_i$ to denote totoal degree
%of $i$ in the fractional matching $M_f$.
%
%For each $i$, let $\hat{d}_i \leq d_i$ be the
%largest number that is an integer multiple
%of $1/(\log^* n)^{2\delta/3}$.
%We shall first slightly scale down the fractional
%matching $M_f$ and get another fractional matching
%$\tilde{M}_f$, such that
%the degree $\tilde{d}_i$ of each supernode $i$
%in $\tilde{M}_f$ is at most $\hat{d}_i$.
%
%\begin{claim}
%There exists a fractional matching $\tilde{M}_f$ in the meta graph
%$H$ such that
%\begin{enumerate}
%    \item The degree $\tilde{d}_i$ of each supernode $i$
%in $\tilde{M}_f$ satisfies $\tilde{d}_i\leq \hat{d}_i$.
%\item The size of $\tilde{M}_f$ satisfies
%$|\tilde{M}_f| \geq |M_f| - k / (log^*n)^{2\delta/3}$.
%\end{enumerate}
%\end{claim}
%
%We then use the trick of spliting each supernode
%$i$ into $\hat{d}_i (\log^* n)^{2\delta/3}$ copies.
%We also split the edges accordingly
%and obtain a fractional matching in the new graph
%so that each copy of each vertex
%has degree at most $1/(\log^* n)^{2\delta/3}$ in the fractional
%matching.
%
%\end{proof}


\subsection{From Amortized to Worst-case}

We now show how to make the update time worst-case
without blowing up the update time by more than a constant factor.

In the sparse regime,
our update time is already worst-case as guaranteed
by the Gupta-Peng algorithm.
We then consider how to make the update time worst-case in the dense regime.

First note that the running time of our algorithm for the dense regime does not
depend on the number of edges.
Thus we could always run the dense regime algorithm in the background,
and only adopt its solution when the graph is dense.
To make the update time worst-case,
we distribute the computation of a $\gamma$-regular partition evenly over
the following $n^{\omega-1}\log^2 n$ updates,
and then distribute the initialization of the data structure with edges $F$
evenly across the $n^{\omega-1}\log^2 n$ updates after.
Of course, at this point the data structure will be falling behind
by $2n^{\omega-1}\log^2 n$ updates. We will then catch it up
in the following $n^{\omega-1}\log^2 n$ updates, by feeding
it $3$ updates per update.
At any point, we will always use the data structure that is up-to-date,
and discard it as soon as a new data structure has become up-to-date.
This way any data structure only goes through $O(n^{\omega-1}\log^2n) $ updates.

Note that we still have to address the switch from the dense regime to sparse regime,
where we restart the Gupta-Peng algorithm by initiating the data structure with the edges
of the entire current graph.
To this end, we actually also always run the Gupta-Peng algorithm in the background,
and only use its solution if needed. But since the running time of the algorithm depends
on the number of edges, we will make sure that the number of edges in the data structure is always
bounded by $n^2 (\log^*n)^{-\delta/8}$.
Specifically, upon the insertion of an edge $e$, if the number of edges in the data structure is
already $n^2 (\log^*n)^{-\delta/8}$, we do not insert $e$ into the data structure,
but store $e$ in a linked list $L$.
Upon the deletion of an edge $e$,
if it is currently in the data structure,
we delete it from the data structure;
otherwise we delete it from $L$.
Moreover,
whenever the number of edges in the data structure becomes strictly
less than $n^2 (\log^*n)^{-\delta/8}$ after a deletion,
we immediately insert an edge in $L$ (if any) into the data structure,
and delete that edge from $L$.
This way, in the sparse regime, it is guaranteed that all edges are in the data structure.


